Machine Learning for Mini-EUSO Telescope Data Analysis

Neural networks as well as other methods of machine learning (ML) are known to be highly efficient in different classification tasks, including classification of images and videos. Mini- EUSO is a wide-field-of-view imaging telescope that operates onboard the International Space Station since 2019 collecting data on miscellaneous processes that take place in the atmosphere of Earth in the UV range. Here we briefly present our results on the development of ML-based approaches for recognition and classification of track-like signals in the Mini-EUSO data, among them meteors, space debris and signals the light curves and kinematics of which are similar to those expected from extensive air showers generated by ultra-high-energy cosmic rays. We show that even simple neural networks demonstrate impressive performance in solving these tasks.

==> JEM-EUSO_Authors_July2023.tex <==
\clearpage
\section*{Full Authors List: The JEM-EUSO Collaboration}
%{\scriptsize (author-list as of July 1st, 2023)} \hspace{0.6cm}
%{\scriptsize (version  \today{} \currenttime{})}
%\vspace*{0.5cm}

\begin{sloppypar}
{\small \noindent
S.~Abe$^{fq}$, 
J.H.~Adams Jr.$^{pd}$, 
D.~Allard$^{cb}$,
P.~Alldredge$^{pd}$,
L.~Anchordoqui$^{pe}$,
A.~Anzalone$^{eh,ed}$, 
E.~Arnone$^{ek,el}$,
M.~Bagheri$^{ph}$,
B.~Baret$^{cb}$,
D.~Barghini$^{el,ek}$,
M.~Battisti$^{ek,el,cb}$,
R.~Bellotti$^{ea,eb}$, 
A.A.~Belov$^{kb}$, 
M.~Bertaina$^{ek,el}$,
P.F.~Bertone$^{pf}$,
M.~Bianciotto$^{ek,el}$,
P.L.~Biermann$^{db}$,
F.~Bisconti$^{ei}$, 
C.~Blaksley$^{ft}$, 
S.~Blin-Bondil$^{cb}$, 
K.~Bolmgren$^{na}$,
S.~Briz$^{pb}$,
J.~Burton$^{pd}$,
F.~Cafagna$^{ea.eb}$, 
G.~Cambi\'e$^{ei,ej}$,
D.~Campana$^{ef}$, 
F.~Capel$^{de}$, 
R.~Caruso$^{ec,ed}$, 
M.~Casolino$^{ft,ei,ej}$,
C.~Cassardo$^{ek,el}$, 
A.~Castellina$^{ek,em}$,
K.~\v{C}ern\'{y}$^{bb}$,  
M.J.~Christl$^{pf}$, 
R.~Colalillo$^{ef,eg}$,
L.~Conti$^{en,ei}$, 
G.~Cotto$^{ek,el}$, 
H.J.~Crawford$^{pa}$, 
R.~Cremonini$^{el}$,
A.~Creusot$^{cb}$, 
A.~de Castro G\'onzalez$^{pb}$,  
C.~de la Taille$^{ca}$, 
R.~Diesing$^{pb}$,
P.~Dinaucourt$^{ca}$,
A.~Di Nola$^{eg}$,
A.~Ebersoldt$^{db}$,
T.~Ebisuzaki$^{ft}$,
J.~Eser$^{pb}$,
F.~Fenu$^{eo}$, 
S.~Ferrarese$^{ek,el}$,
G.~Filippatos$^{pc}$, 
W.W.~Finch$^{pc}$,
F. Flaminio$^{eg}$,
C.~Fornaro$^{en,ei}$,
D.~Fuhne$^{pc}$,
C.~Fuglesang$^{na}$, 
M.~Fukushima$^{fe}$, 
S.~Gadamsetty$^{ph}$,
D.~Gardiol$^{ek,em}$,
G.K.~Garipov$^{kb}$, 
E.~Gazda$^{ph}$, 
A.~Golzio$^{ek,el}$,
F.~Guarino$^{ef,eg}$, 
C.~Gu\'epin$^{pb}$,
A.~Haungs$^{db}$,
T.~Heibges$^{pc}$,
F.~Isgr\`o$^{ef,eg}$, 
E.G.~Judd$^{pa}$, 
F.~Kajino$^{ff}$, 
I.~Kaneko$^{ft}$, 
M.~Kleifges$^{db}$,
P.A.~Klimov$^{kb}$,
I.~Kreykenbohm$^{da}$, 
J.F.~Krizmanic$^{pj}$, 
V.~Kungel$^{pc}$,  
E.~Kuznetsov$^{pd}$, 
F.~L\'opez~Mart\'inez$^{pb}$, 
D.~Mand\'{a}t$^{bc}$,
M.~Manfrin$^{ek,el}$,
A. Marcelli$^{ej}$,
L.~Marcelli$^{ei}$, 
W.~Marsza{\l}$^{ia}$, 
J.N.~Matthews$^{pg}$, 
A.~Menshikov$^{db}$,
M.~Mese$^{ef,eg}$, 
S.S.~Meyer$^{pb}$,
J.~Mimouni$^{ad}$, 
H.~Miyamoto$^{ek,el}$, 
Y.~Mizumoto$^{fi}$,
A.~Monaco$^{ea,eb}$, 
S.~Nagataki$^{ft}$, 
J.~M.~Nachtman$^{pi}$,
D.~Naumov$^{ka}$,
A.~Neronov$^{cb}$,  
T.~Nonaka$^{fe}$, 
T.~Ogawa$^{ft}$, 
S.~Ogio$^{ft}$, 
H.~Ohmori$^{ft}$, 
A.V.~Olinto$^{pb}$,
Y.~Onel$^{pi}$,
G.~Osteria$^{ef}$,  
A.N.~Otte$^{ph}$,  
A.~Pagliaro$^{eh,ed}$,  
B.~Panico$^{ef, eg}$,  
E.~Parizot$^{cb, cd}$, 
I.H.~Park$^{gb}$, 
T.~Paul$^{pe}$,
M.~Pech$^{bc}$, 
F.~Perfetto$^{ef}$,  
P.~Picozza$^{ei,ej}$, 
L.W.~Piotrowski$^{ib}$,
Z.~Plebaniak$^{ei, ej}$, 
J.~Posligua$^{pi}$,
M.~Potts$^{ph}$,
R.~Prevete$^{ef,eg}$,
G.~Pr\'ev\^ot$^{cb}$,
M.~Przybylak$^{ia}$, 
E.~Reali$^{ei, ej}$,
P.~Reardon$^{pd}$, 
M.H.~Reno$^{pi}$, 
M.~Ricci$^{ee}$, 
O.F.~Romero~Matamala$^{ph}$, 
G.~Romoli$^{ei, ej}$,
H.~Sagawa$^{fe}$, 
N.~Sakaki$^{ft}$, 
A.~Santangelo$^{dd}$, 
O.A.~Saprykin$^{kc}$,
F.~Sarazin$^{pc}$,
M.~Sato$^{fo}$, 
H.~Schieler$^{db}$,
P.~Schov\'{a}nek$^{bc}$,
V.~Scotti$^{ef,eg}$,
S.~Selmane$^{cb}$
S.A.~Sharakin$^{kb}$,
K.~Shinozaki$^{ia}$, 
S.~Stepanoff$^{ph}$,
J.F.~Soriano$^{pe}$,
J.~Szabelski$^{ia}$,
N.~Tajima$^{ft}$, 
T.~Tajima$^{ft, pn}$,
Y.~Takahashi$^{fo}$, 
M.~Takeda$^{fe}$, 
Y.~Takizawa$^{ft}$, 
C.~Tenzer$^{dd}$,
S.B.~Thomas$^{pg}$, 
L.G.~Tkachev$^{ka}$,
T.~Tomida$^{fh}$, 
S.~Toscano$^{ob}$,  
M.~Tra\"{i}che$^{aa}$,  
D.~Trofimov$^{cb,kb}$,
K.~Tsuno$^{ft}$,  
P.~Vallania$^{ek,em}$,
L.~Valore$^{ef,eg}$,
T.~M.~Venters$^{pj}$,
C.~Vigorito$^{ek,el}$, 
M.~Vrabel$^{ia}$, 
S.~Wada$^{ft}$,  
J.~Watts~Jr.$^{pd}$, 
A.~Weindl$^{db}$,
L.~Wiencke$^{pc}$, 
J.~Wilms$^{da}$,
D.~Winn$^{pm}$,
H.~Wistrand$^{pc}$,
I.V.~Yashin$^{kb}$, 
R.~Young$^{pf}$,
M.Yu.~Zotov$^{kb}$.
}
\end{sloppypar}
\vspace*{.3cm}

%%\newpage
{ \footnotesize
\noindent
% Algeria - 2 institutes
$^{aa}$ Centre for Development of Advanced Technologies (CDTA), Algiers, Algeria \\
$^{ad}$ Lab. of Math. and Sub-Atomic Phys. (LPMPS), Univ. Constantine I, Constantine, Algeria \\
% Czech Republic - 2 institutes
$^{bb}$ Joint Laboratory of Optics, Faculty of Science, Palack\'{y} University, Olomouc, Czech Republic\\
$^{bc}$ Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic\\
% France - 3 institutes  
$^{ca}$ Omega, Ecole Polytechnique, CNRS/IN2P3, Palaiseau, France\\
$^{cb}$ Universit\'e de Paris, CNRS, AstroParticule et Cosmologie, F-75013 Paris, France\\
$^{cd}$ Institut universitaire de France (IUF)\\
% Germany - 4 institutes
$^{da}$ ECAP, University of Erlangen-Nuremberg, Germany\\
$^{db}$ Karlsruhe Institute of Technology (KIT), Germany\\
$^{dd}$ Institute for Astronomy and Astrophysics, Kepler Center, University of T\"ubingen, Germany\\
$^{de}$ Max Planck Institute for Physics, Munich, Germany\\
% Italy - 15 institutes  
$^{ea}$ Istituto Nazionale di Fisica Nucleare - Sezione di Bari, Italy\\
$^{eb}$ Universita' degli Studi di Bari Aldo Moro and INFN - Sezione di Bari, Italy\\
$^{ec}$ Dipartimento di Fisica e Astronomia "Ettore Majorana", Universita' di Catania, Italy\\
$^{ed}$ Istituto Nazionale di Fisica Nucleare - Sezione di Catania, Italy\\
$^{ee}$ Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, Italy\\
$^{ef}$ Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Italy\\
$^{eg}$ Universita' di Napoli Federico II - Dipartimento di Fisica "Ettore Pancini", Italy\\
$^{eh}$ INAF - Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy\\
$^{ei}$ Istituto Nazionale di Fisica Nucleare - Sezione di Roma Tor Vergata, Italy\\
$^{ej}$ Universita' di Roma Tor Vergata - Dipartimento di Fisica, Roma, Italy\\
$^{ek}$ Istituto Nazionale di Fisica Nucleare - Sezione di Torino, Italy\\
$^{el}$ Dipartimento di Fisica, Universita' di Torino, Italy\\
$^{em}$ Osservatorio Astrofisico di Torino, Istituto Nazionale di Astrofisica, Italy\\
$^{en}$ Uninettuno University, Rome, Italy\\
$^{eo}$ Agenzia Spaziale Italiana, Via del Politecnico, 00133, Roma, Italy\\
% Japan - 7 institutes 
$^{fe}$ Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Japan\\ 
$^{ff}$ Konan University, Kobe, Japan\\ 
$^{fh}$ Shinshu University, Nagano, Japan \\
$^{fi}$ National Astronomical Observatory, Mitaka, Japan\\ 
$^{fo}$ Hokkaido University, Sapporo, Japan \\ 
$^{fq}$ Nihon University Chiyoda, Tokyo, Japan\\ 
$^{ft}$ RIKEN, Wako, Japan\\
% Korea - 1 institute
$^{gb}$ Sungkyunkwan University, Seoul, Republic of Korea\\
% Poland - 2 institutes
$^{ia}$ National Centre for Nuclear Research, Otwock, Poland\\
$^{ib}$ Faculty of Physics, University of Warsaw, Poland\\
% Russia - 3 institutes 
$^{ka}$ Joint Institute for Nuclear Research, Dubna, Russia\\
$^{kb}$ Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Russia\\
$^{kc}$ Space Regatta Consortium, Korolev, Russia\\
% Sweden - 1 institute 
$^{na}$ KTH Royal Institute of Technology, Stockholm, Sweden\\
% Switzerland - 1 institute 
$^{ob}$ ISDC Data Centre for Astrophysics, Versoix, Switzerland\\
% USA - 12 institutes 
$^{pa}$ Space Science Laboratory, University of California, Berkeley, CA, USA\\
$^{pb}$ University of Chicago, IL, USA\\
$^{pc}$ Colorado School of Mines, Golden, CO, USA\\
$^{pd}$ University of Alabama in Huntsville, Huntsville, AL; USA\\
$^{pe}$ Lehman College, City University of New York (CUNY), NY, USA\\
$^{pf}$ NASA Marshall Space Flight Center, Huntsville, AL, USA\\
$^{pg}$ University of Utah, Salt Lake City, UT, USA\\
$^{ph}$ Georgia Institute of Technology, USA\\
$^{pi}$ University of Iowa, Iowa City, IA, USA\\
$^{pj}$ NASA Goddard Space Flight Center, Greenbelt, MD, USA\\
$^{pm}$ Fairfield University, Fairfield, CT, USA\\
$^{pn}$ Department of Physics and Astronomy, University of California, Irvine \\
}


==> JEM-EUSO_Authors_July2023_final.tex <==
\newpage
{\Large\bf Full Authors list: The JEM-EUSO Collaboration\\}
%{\scriptsize (author-list as of July 15th, 2023 with reorganized affiliations)} \hspace{0.6cm}
%{\scriptsize (version  \today{} \currenttime{})}
%\vspace*{0.5cm}

\begin{sloppypar}
{\small \noindent
S.~Abe$^{ff}$, 
J.H.~Adams Jr.$^{ld}$, 
D.~Allard$^{cb}$,
P.~Alldredge$^{ld}$,
R.~Aloisio$^{ep}$,
L.~Anchordoqui$^{le}$,
A.~Anzalone$^{ed,eh}$, 
E.~Arnone$^{ek,el}$,
M.~Bagheri$^{lh}$,
B.~Baret$^{cb}$,
D.~Barghini$^{ek,el}$,
M.~Battisti$^{cb,ek,el}$,
R.~Bellotti$^{ea,eb}$, 
A.A.~Belov$^{ib}$, 
M.~Bertaina$^{ek,el}$,
P.F.~Bertone$^{lf}$,
M.~Bianciotto$^{ek,el}$,
F.~Bisconti$^{ei}$, 
C.~Blaksley$^{fg}$, 
S.~Blin-Bondil$^{cb}$, 
K.~Bolmgren$^{ja}$,
S.~Briz$^{lb}$,
J.~Burton$^{ld}$,
F.~Cafagna$^{ea.eb}$, 
G.~Cambi\'e$^{ei,ej}$,
D.~Campana$^{ef}$, 
F.~Capel$^{db}$, 
R.~Caruso$^{ec,ed}$, 
M.~Casolino$^{ei,ej,fg}$,
C.~Cassardo$^{ek,el}$, 
A.~Castellina$^{ek,em}$,
K.~\v{C}ern\'{y}$^{ba}$,  
M.J.~Christl$^{lf}$, 
R.~Colalillo$^{ef,eg}$,
L.~Conti$^{ei,en}$, 
G.~Cotto$^{ek,el}$, 
H.J.~Crawford$^{la}$, 
R.~Cremonini$^{el}$,
A.~Creusot$^{cb}$,
A.~Cummings$^{lm}$,
A.~de Castro G\'onzalez$^{lb}$,  
C.~de la Taille$^{ca}$, 
R.~Diesing$^{lb}$,
P.~Dinaucourt$^{ca}$,
A.~Di Nola$^{eg}$,
T.~Ebisuzaki$^{fg}$,
J.~Eser$^{lb}$,
F.~Fenu$^{eo}$, 
S.~Ferrarese$^{ek,el}$,
G.~Filippatos$^{lc}$, 
W.W.~Finch$^{lc}$,
F. Flaminio$^{eg}$,
C.~Fornaro$^{ei,en}$,
D.~Fuehne$^{lc}$,
C.~Fuglesang$^{ja}$, 
M.~Fukushima$^{fa}$, 
S.~Gadamsetty$^{lh}$,
D.~Gardiol$^{ek,em}$,
G.K.~Garipov$^{ib}$, 
E.~Gazda$^{lh}$, 
A.~Golzio$^{ek,el}$,
F.~Guarino$^{ef,eg}$, 
C.~Gu\'epin$^{lb}$,
A.~Haungs$^{da}$,
T.~Heibges$^{lc}$,
F.~Isgr\`o$^{ef,eg}$, 
E.G.~Judd$^{la}$, 
F.~Kajino$^{fb}$, 
I.~Kaneko$^{fg}$,
S.-W.~Kim$^{ga}$,
P.A.~Klimov$^{ib}$,
J.F.~Krizmanic$^{lj}$, 
V.~Kungel$^{lc}$,  
E.~Kuznetsov$^{ld}$, 
F.~L\'opez~Mart\'inez$^{lb}$, 
D.~Mand\'{a}t$^{bb}$,
M.~Manfrin$^{ek,el}$,
A. Marcelli$^{ej}$,
L.~Marcelli$^{ei}$, 
W.~Marsza{\l}$^{ha}$, 
J.N.~Matthews$^{lg}$, 
M.~Mese$^{ef,eg}$, 
S.S.~Meyer$^{lb}$,
J.~Mimouni$^{ab}$, 
H.~Miyamoto$^{ek,el}$, 
Y.~Mizumoto$^{fd}$,
A.~Monaco$^{ea,eb}$, 
S.~Nagataki$^{fg}$, 
J.M.~Nachtman$^{li}$,
D.~Naumov$^{ia}$,
A.~Neronov$^{cb}$,  
T.~Nonaka$^{fa}$, 
T.~Ogawa$^{fg}$, 
S.~Ogio$^{fg}$, 
H.~Ohmori$^{fg}$, 
A.V.~Olinto$^{lb}$,
Y.~Onel$^{li}$,
G.~Osteria$^{ef}$,  
A.N.~Otte$^{lh}$,  
A.~Pagliaro$^{ed,eh}$,  
B.~Panico$^{ef,eg}$,  
E.~Parizot$^{cb,cc}$, 
I.H.~Park$^{gb}$, 
T.~Paul$^{le}$,
M.~Pech$^{bb}$, 
F.~Perfetto$^{ef}$,  
P.~Picozza$^{ei,ej}$, 
L.W.~Piotrowski$^{hb}$,
Z.~Plebaniak$^{ei,ej}$, 
J.~Posligua$^{li}$,
M.~Potts$^{lh}$,
R.~Prevete$^{ef,eg}$,
G.~Pr\'ev\^ot$^{cb}$,
M.~Przybylak$^{ha}$, 
E.~Reali$^{ei, ej}$,
P.~Reardon$^{ld}$, 
M.H.~Reno$^{li}$, 
M.~Ricci$^{ee}$, 
O.F.~Romero~Matamala$^{lh}$, 
G.~Romoli$^{ei, ej}$,
H.~Sagawa$^{fa}$, 
N.~Sakaki$^{fg}$, 
O.A.~Saprykin$^{ic}$,
F.~Sarazin$^{lc}$,
M.~Sato$^{fe}$, 
P.~Schov\'{a}nek$^{bb}$,
V.~Scotti$^{ef,eg}$,
S.~Selmane$^{cb}$,
S.A.~Sharakin$^{ib}$,
K.~Shinozaki$^{ha}$, 
S.~Stepanoff$^{lh}$,
J.F.~Soriano$^{le}$,
J.~Szabelski$^{ha}$,
N.~Tajima$^{fg}$, 
T.~Tajima$^{fg, ll}$,
Y.~Takahashi$^{fe}$, 
M.~Takeda$^{fa}$, 
Y.~Takizawa$^{fg}$, 
S.B.~Thomas$^{lg}$, 
L.G.~Tkachev$^{ia}$,
T.~Tomida$^{fc}$, 
S.~Toscano$^{ka}$,  
M.~Tra\"{i}che$^{aa}$,  
D.~Trofimov$^{cb,ib}$,
K.~Tsuno$^{fg}$,  
P.~Vallania$^{ek,em}$,
L.~Valore$^{ef,eg}$,
T.M.~Venters$^{lj}$,
C.~Vigorito$^{ek,el}$, 
M.~Vrabel$^{ha}$, 
S.~Wada$^{fg}$,  
J.~Watts~Jr.$^{ld}$, 
L.~Wiencke$^{lc}$, 
D.~Winn$^{lk}$,
H.~Wistrand$^{lc}$,
I.V.~Yashin$^{ib}$, 
R.~Young$^{lf}$,
M.Yu.~Zotov$^{ib}$.
}
\end{sloppypar}
\vspace*{.3cm}

%%\newpage
{ \footnotesize
\noindent
% Algeria - 2 institutes
$^{aa}$ Centre for Development of Advanced Technologies (CDTA), Algiers, Algeria \\
$^{ab}$ Lab. of Math. and Sub-Atomic Phys. (LPMPS), Univ. Constantine I, Constantine, Algeria \\
% Czech Republic - 2 institutes
$^{ba}$ Joint Laboratory of Optics, Faculty of Science, Palack\'{y} University, Olomouc, Czech Republic\\
$^{bb}$ Institute of Physics of the Czech Academy of Sciences, Prague, Czech Republic\\
% France - 3 institutes  
$^{ca}$ Omega, Ecole Polytechnique, CNRS/IN2P3, Palaiseau, France\\
$^{cb}$ Universit\'e de Paris, CNRS, AstroParticule et Cosmologie, F-75013 Paris, France\\
$^{cc}$ Institut Universitaire de France (IUF), France\\
% Germany - 2 institutes
$^{da}$ Karlsruhe Institute of Technology (KIT), Germany\\
$^{db}$ Max Planck Institute for Physics, Munich, Germany\\
% Italy - 16 institutes  
$^{ea}$ Istituto Nazionale di Fisica Nucleare - Sezione di Bari, Italy\\
$^{eb}$ Universit\`a degli Studi di Bari Aldo Moro, Italy\\
$^{ec}$ Dipartimento di Fisica e Astronomia "Ettore Majorana", Universit\`a di Catania, Italy\\
$^{ed}$ Istituto Nazionale di Fisica Nucleare - Sezione di Catania, Italy\\
$^{ee}$ Istituto Nazionale di Fisica Nucleare - Laboratori Nazionali di Frascati, Italy\\
$^{ef}$ Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Italy\\
$^{eg}$ Universit\`a di Napoli Federico II - Dipartimento di Fisica "Ettore Pancini", Italy\\
$^{eh}$ INAF - Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy\\
$^{ei}$ Istituto Nazionale di Fisica Nucleare - Sezione di Roma Tor Vergata, Italy\\
$^{ej}$ Universit\`a di Roma Tor Vergata - Dipartimento di Fisica, Roma, Italy\\
$^{ek}$ Istituto Nazionale di Fisica Nucleare - Sezione di Torino, Italy\\
$^{el}$ Dipartimento di Fisica, Universit\`a di Torino, Italy\\
$^{em}$ Osservatorio Astrofisico di Torino, Istituto Nazionale di Astrofisica, Italy\\
$^{en}$ Uninettuno University, Rome, Italy\\
$^{eo}$ Agenzia Spaziale Italiana, Via del Politecnico, 00133, Roma, Italy\\
$^{ep}$ Gran Sasso Science Institute, L'Aquila, Italy\\
% Japan - 7 institutes 
$^{fa}$ Institute for Cosmic Ray Research, University of Tokyo, Kashiwa, Japan\\ 
$^{fb}$ Konan University, Kobe, Japan\\ 
$^{fc}$ Shinshu University, Nagano, Japan \\
$^{fd}$ National Astronomical Observatory, Mitaka, Japan\\ 
$^{fe}$ Hokkaido University, Sapporo, Japan \\ 
$^{ff}$ Nihon University Chiyoda, Tokyo, Japan\\ 
$^{fg}$ RIKEN, Wako, Japan\\
% Korea - 2 institutes
$^{ga}$ Korea Astronomy and Space Science Institute\\
$^{gb}$ Sungkyunkwan University, Seoul, Republic of Korea\\
% Poland - 2 institutes
$^{ha}$ National Centre for Nuclear Research, Otwock, Poland\\
$^{hb}$ Faculty of Physics, University of Warsaw, Poland\\
% Russia - 3 institutes 
$^{ia}$ Joint Institute for Nuclear Research, Dubna, Russia\\
$^{ib}$ Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, Russia\\
$^{ic}$ Space Regatta Consortium, Korolev, Russia\\
% Sweden - 1 institute 
$^{ja}$ KTH Royal Institute of Technology, Stockholm, Sweden\\
% Switzerland - 1 institute 
$^{ka}$ ISDC Data Centre for Astrophysics, Versoix, Switzerland\\
% USA - 13 institutes 
$^{la}$ Space Science Laboratory, University of California, Berkeley, CA, USA\\
$^{lb}$ University of Chicago, IL, USA\\
$^{lc}$ Colorado School of Mines, Golden, CO, USA\\
$^{ld}$ University of Alabama in Huntsville, Huntsville, AL, USA\\
$^{le}$ Lehman College, City University of New York (CUNY), NY, USA\\
$^{lf}$ NASA Marshall Space Flight Center, Huntsville, AL, USA\\
$^{lg}$ University of Utah, Salt Lake City, UT, USA\\
$^{lh}$ Georgia Institute of Technology, USA\\
$^{li}$ University of Iowa, Iowa City, IA, USA\\
$^{lj}$ NASA Goddard Space Flight Center, Greenbelt, MD, USA\\
$^{lk}$ Fairfield University, Fairfield, CT, USA\\
$^{ll}$ Department of Physics and Astronomy, University of California, Irvine, USA \\
$^{lm}$ Pennsylvania State University, PA, USA \\
}


